Learning Heterogeneous Performance-Fairness Trade-offs in Federated Learning

Recent methods leverage a hypernet to handle the performance-fairness trade-offs in federated learning. This hypernet maps the clients' preferences between model performance and fairness to preference-specifc models on the trade-off curve, known as local Pareto front. However, existing methods typically adopt a uniform preference sampling distribution to train the hypernet across clients, neglecting the inherent heterogeneity of their local Pareto fronts. Meanwhile, from the perspective of generalization, they do not consider the gap between local and global Pareto fronts on the global dataset. To address these limitations, we propose HetPFL to effectively learn both local and global Pareto fronts. HetPFL comprises Preference Sampling Adaptation (PSA) and Preference-aware Hypernet Fusion (PHF). PSA adaptively determines the optimal preference sampling distribution for each client to accommodate heterogeneous local Pareto fronts. While PHF performs preference-aware fusion of clients' hypernets to ensure the performance of the global Pareto front. We prove that HetPFL converges linearly with respect to the number of rounds, under weaker assumptions than existing methods. Extensive experiments on four datasets show that HetPFL significantly outperforms seven baselines in terms of the quality of learned local and global Pareto fronts.

==> Section/problem.tex <==
\section{Problem Formulation}



% \subsubsection{Challenges}
% In the context of FL, learning the Pareto frontier faces various challenges that previous works have not considered.
% \begin{enumerate}[label=(\arabic*)]
%     \item Pareto front of clients are heterogeneous. As shown in Fig. \ref{sampling}, the preference sampling distribution of each client needs to be adapted according to the location of the Pareto front.
%     \item Eq. (\ref{local}) only focuses on the local Pareto front of clients, which ignores the performance of the Pareto front on the global dataset. However, both the local Pareto front and the global Pareto front are important.
% \end{enumerate}
